A Methodology to Select Topology Generators for WANET Simulations (Extended Version)

Many academic and industrial research works on WANETs rely on simulations, at least in the first stages, to obtain preliminary results to be subsequently validated in real settings. Topology generators (TG) are commonly used to generate the initial placement of nodes in artificial WANET topologies, where those simulations take place. The significance of these experiments heavily depends on the representativeness of artificial topologies. Indeed, if they were not drawn fairly, obtained results would apply only to a subset of possible configurations, hence they would lack of the appropriate generality required to port them to the real world. Although using many TGs could mitigate this issue by generating topologies in several different ways, that would entail a significant additional effort. Hence, the problem arises of what TGs to choose, among a number of available generators, to maximise the representativeness of generated topologies and reduce the number of TGs to use. In this paper, we address that problem by investigating the presence of bias in the initial placement of nodes in artificial WANET topologies produced by different TGs. We propose a methodology to assess such bias and introduce two metrics to quantify the diversity of the topologies generated by a TG with respect to all the available TGs, which can be used to select what TGs to use. We carry out experiments on three well-known TGs, namely BRITE, NPART and GT-ITM. Obtained results show that using the artificial networks produced by a single TG can introduce bias.

==> discussion.tex <==
\section{Discussion} \label{s:discussion}
  
Visual inspection of the topologies from the NPART, BRITE and GT-ITM generators seemed identical. Taking the class agnostic algorithm results gave a result of an optimum value of 2 classes. When given the correct number of classes to the analysis, it gave a best accuracy of 67\%, which increases to an accuracy of 72\% when the probabilistic algorithms and were trained on a proportion of the data. Using the sequential feature selection (SFS) this gave a final accuracy of 78.6\%, this cannot be rated as very accurate.

The way the supervised learning techniques is used splits the data into train and testing parts. Once trained, predictions are made on the test data, it was though interesting to see how the wrongly predicted values were distributed. It was shown that not all three classes were misclassified evenly.

The BRITE class was always classified correctly, while NPART and GT-ITM made up the error, almost equally split between these two classes.
To get clearer results, the analysis was then broken down into paired comparisons. This showed that BRITE could be distinguished from either of the other two classes with 100\% accuracy while NPART and GTITM gave a maximum of 64\% accuracy, increasing to 77\% when applying SFS.

Again SFS was used to find the best combination of features. This showed that the “Clustering coefficient with radius of 20 units” by itself explained all the variance when comparing BRITE vs NPART and BRITE vs GT-ITM. While greatest accuracy for NPART vs GT-ITM was explained by "Inter-node distance feature - Mode of euclidean distance"

